Accelerating Image Super-Resolution Networks with Pixel-Level Classification

In recent times, the need for effective super-resolution (SR) techniques has surged, especially for large-scale images ranging 2K to 8K resolutions. For DNN-based SISR, decomposing images into overlapping patches is typically necessary due to computational constraints. In such patch-decomposing scheme, one can allocate computational resources differently based on each patch's difficulty to further improve efficiency while maintaining SR performance. However, this approach has a limitation: computational resources is uniformly allocated within a patch, leading to lower efficiency when the patch contain pixels with varying levels of restoration difficulty. To address the issue, we propose the Pixel-level Classifier for Single Image Super-Resolution (PCSR), a novel method designed to distribute computational resources adaptively at the pixel level. A PCSR model comprises a backbone, a pixel-level classifier, and a set of pixel-level upsamplers with varying capacities. The pixel-level classifier assigns each pixel to an appropriate upsampler based on its restoration difficulty, thereby optimizing computational resource usage. Our method allows for performance and computational cost balance during inference without re-training. Our experiments demonstrate PCSR's advantage over existing patch-distributing methods in PSNR-FLOP trade-offs across different backbone models and benchmarks. The code is available at https://github.com/3587jjh/PCSR.

==> main/partials/fig_comparisons_.tex <==
\begin{figure}[]
\centering
\tiny
\begin{tabular}
{@{}m{0.35\linewidth}@{\hskip2pt}m{0.15\linewidth}@{\hskip2pt}m{0.15\linewidth}@{\hskip2pt}m{0.15\linewidth}@{\hskip2pt}m{0.15\linewidth}@{}}

% 2
\multirow{3}{*}{\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_001_010_y512_x000_Box}} &
\centering{ClassSR 24.77dB/50.9G(92\%)} &
\centering{ARM 24.76dB/50.4G(91\%)} &
\centering{Ours 24.93dB/37.8G(68\%)} &
\centering{CARN 25.00dB/55.5G(100\%)} \tabularnewline
&
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_001_010_y512_x000_ClassSR} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_001_010_y512_x000_ARM} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_001_010_y512_x000_Ours} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_001_010_y512_x000_CARN} \tabularnewline
&
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_001_010_y512_x000_ClassSR_Colored} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_001_010_y512_x000_ARM_Colored} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_001_010_y512_x000_Ours_Colored} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_001_010_y512_x000_GT} \tabularnewline

%3
\multirow{3}{*}{\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_002_y000_x768_Box}} &
\centering{ClassSR 21.21dB/45.0G(97\%)} &
\centering{ARM 21.09dB/45.4G(98\%)} &
\centering{Ours 21.40dB/33.7G(73\%)} &
\centering{CARN 21.34dB/46.3G(100\%)} \tabularnewline
&
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_002_y000_x768_ClassSR} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_002_y000_x768_ARM} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_002_y000_x768_Ours} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_002_y000_x768_CARN} \tabularnewline
&
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_002_y000_x768_ClassSR_Colored} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_002_y000_x768_ARM_Colored} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_002_y000_x768_Ours_Colored} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_002_y000_x768_GT} \tabularnewline

%4
\multirow{3}{*}{\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_006_y384_x512_Box}} &
\centering~ClassSR (00dB/00G) &
\centering~ARM (00dB/00G) &
\centering~Ours (00dB/00G) &
\centering~CARN (00dB/00G) \tabularnewline
&
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_006_y384_x512_ClassSR} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_006_y384_x512_ARM} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_006_y384_x512_Ours} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_006_y384_x512_CARN} \tabularnewline
&
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_006_y384_x512_ClassSR_Colored} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_006_y384_x512_ARM_Colored} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_006_y384_x512_Ours_Colored} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_006_y384_x512_GT} \tabularnewline

%5
\multirow{3}{*}{\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_010_y384_x384_Box}} &
\centering~ClassSR (00dB/00G) &
\centering~ARM (00dB/00G) &
\centering~Ours (00dB/00G) &
\centering~CARN (00dB/00G) \tabularnewline
&
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_010_y384_x384_ClassSR} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_010_y384_x384_ARM} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_010_y384_x384_Ours} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_010_y384_x384_CARN} \tabularnewline
&
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_010_y384_x384_ClassSR_Colored} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_010_y384_x384_ARM_Colored} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_010_y384_x384_Ours_Colored} &
\includegraphics[width=\linewidth]{main/assets/fig_comparisons1/Urban100_003_010_y384_x384_GT} \tabularnewline
\end{tabular}
\caption{
visual comparisons
}
\label{fig:visual_comparisons}
\end{figure}

==> main/partials/tab_general_application.tex <==
\begin{table}[]
\centering
\caption{
\textcolor{red}{GENERAL APPLICATION} 
% S- and O- represents slots and objects.
}
\label{tab:general_application}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|cc|cc|cc|cc|}
\hline
Models          & Parameters & B100(dB) & GFLOPs     & Urban100(dB) & GFLOPs     & Manga109(dB) & GFLOPs     & Test2K(dB) & GFLOPs      \\ \hline
BSRN            & 352K      & 26.46    & 4.63 (100\%)  & 24.23     & 29.1 (100\%) & 28.31    & 37.7 (100\%) & 26.04        & 66.0 (100\%)  \\
% IMDN-SMSR       & 0.77M      & 32.11    & 7.7 (78\%)   & 28.55     & 15.6. (78\%) & 27.53    & 10.6 (78\%)  & 26.02        & 53.5 (78\%)   \\
% BSRN-PCSR (ours)     & -          & -        & -            & -         & -            & -        & -            & -            & -             \\
BSRN-PCSR (ours)     & 265K          & 26.45        & 3.98 (86\%)            & 24.26         & 24.8 (85\%)            & 28.02        & 31.6 (84\%)            & 26.08            & 57.1 (87\%)             \\ \hline
LBNet        & 742K       & 26.52    & 27.9 (100\%) & 24.46     & 538.9 (100\%) & 28.64    & 835.9 (100\%) & 26.15        & 2445.2 (100\%) \\
% SRResNet-SMSR   & 1.6M       & 32.03    & 20.0 (65\%)  & 28.52     & 40.6 (65\%)  & 27.52    & 27.7 (65\%)  & 25.97        & 139.5 (65\%)  \\
% SRResNet-Ours-1 & -          & -        & -            & -         & -            & -        & -            & -            & -             \\
LBNet-PCSR (ours) & 498K          & 26.47        & 21.2 (76\%)            & 24.46         & 410.7 (76\%)            & 28.34        & 633.9 (76\%)            & 26.09            & 1836.0 (75\%)             \\ \hline
\end{tabular}
}
\end{table}

==> main/partials/tab_main_.tex <==
\begin{table}[]
% \begin{sidewaystable}
\centering
\caption{
The comparison of the previous patch-level methods and our pixel-level method PCSR on the large image SR benchmarks: Test2K, Test4K, Test8K, and Urban 100.
The lowest FLOPs values are highlighted in bold.
}
\label{tab:main}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|cc|cc|cc|cc|}
\hline
Models            & Params. & Test2K(dB)   & GFLOPs         & Test4K(dB)  & GFLOPs          & Test8K(dB)         & GFLOPs           & Urban100(dB) & GFLOPs         \\ \hline
FSRCNN-full      & 25K        & 25.69  & 45 (100\%)  & 26.99  & 185 (100\%)  & 32.82        & 1068 (100\%)  & 23.05  & 20 (100\%)  \\
FSRCNN-classSR   & 113K       & 25.61  & 38 (85\%)   & 26.91  & 146 (79\%)   & 32.73        & 709 (66\%)    & 22.89  & 21 (105\%)  \\
FSRCNN-ARM       & 25K        & 25.61  & 36 (79\%)   & 26.91  & 153 (83\%)   & 32.73        & 747 (70\%)    & 22.89  & 20 (100\%)  \\
% FSRCNN-ours-1    & 39K        & -        & -              & -        & -               & -              & -                & -        & -              \\
FSRCNN-PCSR   & 39K        & 25.61  & \textbf{7.4 (16\%})  & 26.91  &\textbf{ 30 (16\%)}  & 32.74   & \textbf{191 (18\%)}  & 22.90  &\textbf{ 3.2 (16\%)}  \\ \hline
CARN-full        & 295K       & 26.03  & 112 (100\%) & 27.45  & 458 (100\%)  & 33.29   & 2639 (100\%)  & 24.03  & 49 (100\%)  \\
CARN-classSR     & 645K       & 26.01  & 102 (91\%)  & 27.42  & 384 (84\%)   & 33.25        & 1830 (69\%)   & 24.00  & 52(105\%)   \\
CARN-ARM         & 295K       & 26.01  & 100 (89\%)  & 27.42  & 379 (83\%)   & 33.26        & 1783 (68\%)   & 23.99  & 51 (103\%)  \\
% CARN-ours-1      & 171K       & -        & -              & -        & -               & -              & -                & -        & -              \\
CARN-PCSR   & 171K       & 26.01  & \textbf{60 (53\%)}  & 27.42   & \textbf{237 (52\%)}  & 33.26   & \textbf{1329 (50\%)}   & 24.00  & \textbf{28 (56\%)}   \\ \hline
SRResNet-full    & 1.5M       & 26.24  & 503 (100\%) & 27.71  & 2056 (100\%) & 33.55   & 11851 (100\%) & 24.65  & 221 (100\%) \\
SRResNet-classSR & 3.1M       & 26.20  & 446 (89\%)  & 27.66  & 1686 (82\%)  & 33.50        & 7996 (67\%)   & 24.54  & 227 (102\%) \\
SRResNet-ARM     & 1.5M       & 26.20  & 429 (85\%)  & 27.66  & 1742 (85\%)  & 33.50        & 7865 (66\%)   & 24.54  & 245 (111\%) \\
% SRResNet-ours-1  & 1.1M       & -        & -              & -        & -               & -              & -                & -        & -              \\
SRResNet-PCSR  & 1.1M       & 26.20  &\textbf{ 333 (66\%)}  & 27.66  & \textbf{1239 (60\%)}   & 33.50   & \textbf{6860 (58\%)}   & 24.54   & \textbf{134 (61\%)} \\ \hline
\end{tabular}
}
% \end{sidewaystable}
\end{table}
